PaCoRe: Learning to Scale Test-Time Compute with Parallel Coordinated Reasoning

We introduce Parallel Coordinated Reasoning (PaCoRe), a training-and-inference framework designed to overcome a central limitation of contemporary language models: their inability to scale test-time compute (TTC) far beyond sequential reasoning under a fixed context window. PaCoRe departs from the traditional sequential paradigm by driving TTC through massive parallel exploration coordinated via a message-passing architecture in multiple rounds. Each round launches many parallel reasoning trajectories, compacts their findings into context-bounded messages, and synthesizes these messages to guide the next round and ultimately produce the final answer. Trained end-to-end with large-scale, outcome-based reinforcement learning, the model masters the synthesis abilities required by PaCoRe and scales to multi-million-token effective TTC without exceeding context limits. The approach yields strong improvements across diverse domains, and notably pushes reasoning beyond frontier systems in mathematics: an 8B model reaches 94.5% on HMMT 2025, surpassing GPT-5's 93.2% by scaling effective TTC to roughly two million tokens. We open-source model checkpoints, training data, and the full inference pipeline to accelerate follow-up work.

==> commands.tex <==
\newcommand{\lstm}{\textsc{LSTM}}
\newcommand{\ffw} {\textsc{Ffw}}
\newcommand{\attn}{\textsc{Attn}}
\newcommand{\encoder} {\textsc{Encoder}}
\newcommand{\key} {\textsc{Key}}
\newcommand{\query} {\textsc{Query}}
\newcommand{\ccca}{\textsc{Cca}}
\newcommand{\crossattention}{\textsc{Ca}}
\newcommand{\softmax}{\textrm{softmax}}
\newcommand{\ret}{\textsc{Ret}}
\newcommand{\block}{\textsc{Block}}
\newcommand{\MassiveText} {Massive Text}
\newcommand{\bert}{\textsc{Bert}\xspace}
\newcommand{\model}{\textsc{Model}}
\renewcommand{\encoder}{\textsc{Encoder}}
\newcommand{\knnlm}{k\textrm{NN-LM}}
\newcommand{\knn}{k\textrm{NN}}
\newcommand{\spalm}{\textsc{Spalm}}
\newcommand{\dpr}{\textsc{Dpr}}
\newcommand{\rag}{\textsc{RAG}}
\newcommand{\realm}{\textsc{Realm}}
\newcommand{\fid}{\textsc{FiD}}
\newcommand{\emdr}{\textsc{Emdr}^2}
\newcommand{\retro}{\textsc{Retro}\xspace}
\newcommand{\retroon}{\textsc{Retro[On]}\xspace}
\newcommand{\retrooff}{\textsc{Retro[Off]}\xspace}
\newcommand{\retrofit}{\textsc{Retro}fit\xspace}
\newcommand{\retrofitting}{\textsc{Retro}fitting\xspace}
\newcommand{\lm}{\textsc{Lm}}
\newcommand{\lmc}{\textsc{Lmc}}
\newcommand{\emb}{\textsc{Emb}}
\newcommand{\readout}{\textsc{Read}}
\newcommand{\spli}{\textsc{Split}}
\newcommand{\bpb}{\textrm{bpb}}
\newcommand{\dmodel}{d}
\newcommand{\dffw}{d_{\textrm{ffw}}}
\newcommand{\lcp}{\textrm{LCP}}

\newcommand{\datavisheader}[0]{
$C_u$ colored by loss difference & $C_u$ colored by LCP with $\ret(C_u{-1})$  & $[N_u^1, F_u^1]$ colored by LCP with $C_{u+1}$ & $[N_u^2, F_u^2]$ colored by LCP with $C_{u+1}$\\ 
$L_{\textsc{\retrooff}} - L_{\retro}\colorbox{cm_0!40}{$ \leq -0.5$}, \colorbox{cm_31!40}{$=0 $},\colorbox{cm_63!40}{$ \geq 0.5$}$
& $ \lcp = $ \colorbox{cm_0!40}{$0$}, \colorbox{cm_12!40}{$1 $}, \colorbox{cm_25!40}{$2 $}, \colorbox{cm_38!40}{$3 $},\colorbox{cm_51!40}{$4 $},\colorbox{cm_63!40}{$ \geq 5 $} & $ \lcp = $  \colorbox{cm_0!40}{$0$}, \colorbox{cm_12!40}{$1 $}, \colorbox{cm_25!40}{$2 $}, \colorbox{cm_38!40}{$3 $},\colorbox{cm_51!40}{$4 $},\colorbox{cm_63!40}{$ \geq 5 $} &
$ \lcp = $ \colorbox{cm_0!40}{$0$}, \colorbox{cm_12!40}{$1 $}, \colorbox{cm_25!40}{$2 $}, \colorbox{cm_38!40}{$3 $},\colorbox{cm_51!40}{$4 $},\colorbox{cm_63!40}{$ \geq 5 $} \\
\toprule}

\newcommand{\samplevisheader}[0]{
Prompt and sample of $\retrooff$  & Prompt and sample of $\retroon$ & $[N_u^1, F_u^1]$ colored by LCP with $C_{u+1}$ & $[N_u^2, F_u^2]$ colored by LCP with $C_{u+1}$\\ 

& 
colored by LCP with $\ret(C_u{-1})$ 
& & \\

&$ \lcp = $ \colorbox{cm_0!40}{$0$}, \colorbox{cm_12!40}{$1 $}, \colorbox{cm_25!40}{$2 $}, \colorbox{cm_38!40}{$3 $},\colorbox{cm_51!40}{$4 $},\colorbox{cm_63!40}{$ \geq 5 $} & $ \lcp = $  \colorbox{cm_0!40}{$0$}, \colorbox{cm_12!40}{$1 $}, \colorbox{cm_25!40}{$2 $}, \colorbox{cm_38!40}{$3 $},\colorbox{cm_51!40}{$4 $},\colorbox{cm_63!40}{$ \geq 5 $}  &$ \lcp = $ \colorbox{cm_0!40}{$0$}, \colorbox{cm_12!40}{$1 $}, \colorbox{cm_25!40}{$2 $}, \colorbox{cm_38!40}{$3 $},\colorbox{cm_51!40}{$4 $},\colorbox{cm_63!40}{$ \geq 5 $} \\ 

\toprule}


\newcommand{\NN}{\mathbb{N}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\PP}{\mathbb{P}}
\renewcommand{\SS}{\mathbb{S}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\Aa}{\mathcal{A}}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dd}{\mathcal{D}}
\newcommand{\Ee}{\mathcal{E}}
\newcommand{\Ff}{\mathcal{F}}
\newcommand{\Gg}{\mathcal{G}}
\newcommand{\Hh}{\mathcal{H}}
\newcommand{\Ii}{\mathcal{I}}
\newcommand{\Jj}{\mathcal{J}}
\newcommand{\Kk}{\mathcal{K}}
\newcommand{\Ll}{\mathcal{L}}
\newcommand{\Mm}{\mathcal{M}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Oo}{\mathcal{O}}
\newcommand{\Pp}{\mathcal{P}}
\newcommand{\Qq}{\mathcal{Q}}
\newcommand{\Rr}{\mathcal{R}}
\newcommand{\Ss}{\mathcal{S}}
\newcommand{\Tt}{\mathcal{T}}
\newcommand{\Uu}{\mathcal{U}}
\newcommand{\Vv}{\mathcal{V}}
\newcommand{\Ww}{\mathcal{W}}
\newcommand{\Xx}{\mathcal{X}}
\newcommand{\Yy}{\mathcal{Y}}
\newcommand{\Zz}{\mathcal{Z}}



\newcommand{\al}{\alpha}
\newcommand{\la}{\lambda}
\newcommand{\ga}{\gamma}
\newcommand{\Ga}{\Gamma}
\newcommand{\La}{\Lambda}
\newcommand{\si}{\sigma}
\newcommand{\be}{\beta}
\newcommand{\de}{\delta}
\newcommand{\De}{\Delta}
\renewcommand{\phi}{\varphi}
\renewcommand{\th}{\theta}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}

\newcommand{\hf}{\hat f}
\newcommand{\wtf}{\tilde f}
\newcommand{\tx}{\tilde x}
\newcommand{\ta}{\tilde a}
\newcommand{\tb}{\tilde b}
\newcommand{\ty}{\tilde y}
\newcommand{\tu}{\tilde u}
\newcommand{\tv}{\tilde v}
\newcommand{\tga}{\tilde \ga}
\newcommand{\tf}{\wt{f}}



\newcommand{\ins}[1]{\mathrm{#1}}
\let\Re\relax

\DeclareMathOperator{\Re}{\Rr e}
\DeclareMathOperator{\Imag}{\Ii m}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Supp}{Supp}
\DeclareMathOperator{\Sign}{Sign}
\let\Im\relax
\DeclareMathOperator{\Im}{Im}
\DeclareMathOperator{\Corr}{Corr}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\supp}{supp}

\DeclareMathOperator{\cas}{cas}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\cotan}{cotan}
\DeclareMathOperator{\Card}{Card}
\DeclareMathOperator{\GCD}{GCD}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\interop}{int}

\newcommand{\ps}[2]{\langle #1,#2\rangle}

\newcommand{\Calpha}{\mathrm{C}^\al}
\newcommand{\Cbeta}{\mathrm{C}^\be}
\newcommand{\Cal}{\text{C}^\al}
\newcommand{\Ctwo}{\text{C}^{2}}
\newcommand{\Calt}[1]{\text{C}^{#1}}
\newcommand{\Cder}[1]{\mathscr{C}^{#1}}
\newcommand{\lone}{\ell^1}
\newcommand{\ltwo}{\ell^2}
\newcommand{\linf}{\ell^\infty}
\newcommand{\Lone}{\text{\upshape L}^1}
\newcommand{\Ltwo}{\text{\upshape L}^2}
\newcommand{\Linf}{\text{\upshape L}^\infty}
\newcommand{\lzero}{\ell^0}
\newcommand{\lp}{\ell^p}
\newcommand{\Sun}{\text{S}^1}
\newcommand{\foralls}{\forall \,}
\newcommand{\dd}{\ins{d}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}



\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\whwh}[1]{\hat{\hat{#1}}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\pd}[2]{ \frac{ \partial #1}{\partial #2} }
\newcommand{\pdd}[2]{ \frac{ \partial^2 #1}{\partial #2^2} }
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\imath}{\mathrm{i}}
\newcommand{\interior}[1]{\ensuremath{\overset{\circ}{#1}}}

\newcommand{\legsymb}[2]{ \genfrac{(}{)}{}{}{#1}{#2} }
\newcommand{\ordin}[2]{ ${#1}^{ \text{#2} }$ }
\newcommand{\dotp}[2]{\langle #1,\,#2\rangle}
\newcommand{\dotps}[2]{\langle #1,\,#2\rangle}
\newcommand{\crossp}[2]{ #1 \hat #2 }
\newcommand{\seg}[2]{\llbracket #1,\,#2 \rrbracket}
\newcommand{\brac}[1]{\left[#1\right]}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\snorm}[1]{\| #1 \|}
\newcommand{\normb}[1]{\Big|\!\Big| #1 \Big |\!\Big|}
\newcommand{\normB}[1]{\left|\!\left| #1 \right|\!\right|}
\DeclareMathOperator{\diverg}{div}
\DeclareMathOperator{\Prox}{Prox}
\newcommand{\normT}[1]{\norm{#1}_{\text{T}}}
\newcommand{\normu}[1]{\norm{#1}_{1}}
\newcommand{\normi}[1]{\norm{#1}_{\infty}}
\newcommand{\normd}[1]{\norm{#1}_{2}}
\newcommand{\normz}[1]{\norm{#1}_{0}}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert} %
\newcommand{\absb}[1]{\Big| #1 \Big|}

\newcommand{\func}[4]{ {\left\{  \begin{array}{ccc} #1 & \longrightarrow & #2 \\ #3 & \longmapsto & #4 \end{array}  \right.} }
\newcommand{\Id}{\ins{Id}}
\newcommand{\eqdef}{\triangleq}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\newcommand{\pa}[1]{\left( #1 \right)}
\newcommand{\bpa}[1]{\big( #1 \big)}
\newcommand{\choice}[1]{ %
	\left\{ %
		\begin{array}{l} #1 \end{array} %
	\right. }
\newcommand{\set}[1]{ \{ #1 \} }
\newcommand{\condset}[2]{ \left\{ #1 \;;\; #2 \right\} }


\newcommand{\qandq}{ \quad \text{and} \quad }
\newcommand{\qqandqq}{ \qquad \text{and} \qquad }
\newcommand{\qifq}{ \quad \text{if} \quad }
\newcommand{\qqifqq}{ \qquad \text{if} \qquad }
\newcommand{\qwhereq}{ \quad \text{where} \quad }
\newcommand{\qqwhereqq}{ \qquad \text{where} \qquad }
\newcommand{\qwithq}{ \quad \text{with} \quad }
\newcommand{\qqwithqq}{ \qquad \text{with} \qquad }
\newcommand{\qforq}{ \quad \text{for} \quad }
\newcommand{\qqforqq}{ \qquad \text{for} \qquad }
\newcommand{\qqsinceqq}{ \qquad \text{since} \qquad }
\newcommand{\qsinceq}{ \quad \text{since} \quad }
\newcommand{\qarrq}{\quad\Longrightarrow\quad}
\newcommand{\qqarrqq}{\quad\Longrightarrow\quad}
\newcommand{\qiffq}{\quad\Longleftrightarrow\quad}
\newcommand{\qqiffqq}{\qquad\Longleftrightarrow\qquad}
\newcommand{\qsubjq}{ \quad \text{subject to} \quad }
\newcommand{\qqsubjqq}{ \qquad \text{subject to} \qquad }
\newcommand{\qobjq}[1]{\quad \text{#1} \quad}
\newcommand{\qqobjqq}[1]{\quad \text{#1} \quad}





\newlength{\restsubwidth}
\newlength{\restsubheight}
\newlength{\restsubmoreheight}
\setlength{\restsubmoreheight}{4pt}
\newcommand{\rest}[2]{%
        \settowidth{\restsubwidth}{\ensuremath{#2}}
        \settoheight{\restsubheight}{\ensuremath{{}_{#2}}}
        \ensuremath{{#1\hskip 0.5pt}_{\vrule\kern2pt\parbox[b][%
        4pt][b]{\the\restsubwidth}{%
                        \ensuremath{{}_{#2}}}}}
        }

